Pre-train a Discriminative Text Encoder for Dense Retrieval via Contrastive Span Prediction

Dense retrieval has shown promising results in many information retrieval (IR) related tasks, whose foundation is high-quality text representation learning for effective search. Some recent studies have shown that autoencoder-based language models are able to boost the dense retrieval performance using a weak decoder. However, we argue that 1) it is not discriminative to decode all the input texts and, 2) even a weak decoder has the bypass effect on the encoder. Therefore, in this work, we introduce a novel contrastive span prediction task to pre-train the encoder alone, but still retain the bottleneck ability of the autoencoder. % Therefore, in this work, we propose to drop out the decoder and introduce a novel contrastive span prediction task to pre-train the encoder alone. The key idea is to force the encoder to generate the text representation close to its own random spans while far away from others using a group-wise contrastive loss. In this way, we can 1) learn discriminative text representations efficiently with the group-wise contrastive learning over spans and, 2) avoid the bypass effect of the decoder thoroughly. Comprehensive experiments over publicly available retrieval benchmark datasets show that our approach can outperform existing pre-training methods for dense retrieval significantly.

==> background.tex <==
\begin{figure*}
    \centering
    \includegraphics[scale=0.45]{imgs/model.png}
    \caption{SimCDR Overview: A special token is added in front of every document to produce document representations;  Document representations are transformed through a projector which is an MLP with a non-linear function; We sample multiple local spans with different lengths to simulate words, phrases, sentences and paragraphs, and do average pooling to obtain their representations; SimCDR pulls the document representation close with representations of multiple fine-grained spans in the same document and pushes it apart from both the document and span representations of other documents.}
    \label{fig:model}
\end{figure*}


\section{Background}

% \subsection{PROP}
% Our method is built upon PROP~\cite{}, so we would like to first briefly review this method in this section.
% The key idea of PROP is inspired by the traditional statistical language model for IR, specifically the query likelihood model~\cite{}. 
% The query likelihood model assumes that the query $Q$ is generated as a piece of text representative of the ``ideal'' document $D$.
% Such a query-generation idea could then be formulated using the Bayesian theorem:
% \begin{equation}
%  P(D|Q) \propto P(Q|\theta_D)P(D),
% \end{equation}
% where $\theta_D$ is the document language model.
% The prior probability $P(D)$ is usually assumed to be uniform across all documents and thus can be ignored.
% The documents are then ranked by the probability of the document generating the query $P(Q|\theta_D)$.


% Based on this assumption, the representative words prediction (ROP) task is introduced for pre-training for IR as follows.
% Given an input document, a pair of word sets are sampled according to the document language model like a multinomial unigram language model with Dirichlet prior smoothing used in PROP and the contrastive term distribution used in B-PROP.
% Since words within the document usually have higher probabilities than those outside the document, this sampling mostly samples words from the document.
% In addition, words are sampled independently to form a word set, which leads to semantic incompleteness and ambiguity of the word set.
% The word set with higher likelihood is deemed as more ``representative'' of the document. 
% A Transformer model is then pre-trained to predict the pairwise preference between the two sets of words. 


% During pre-training, the word set $s$ and the document $d$ are concatenated  with special delimiter tokens as a single input sequence, i.e., [CLS]+$s$+[SEP]+$d$+[SEP], and fed into the Transformer.  
% Let a triple $(s_1,s_2,d)$ denote the pair of word sets sampled from the corresponding document $d$. 
% The ROP task can be formulated by a typical pairwise loss, i.e., hinge loss, for the pre-training,
% \begin{equation}
% \label{ROP}
% \mathcal{L}_{ROP} = max(0, 1-P(s_1|d)+P(s_2|d)),
% \end{equation}
% where the likelihood of each set $P(s|d)$ denotes how representative the word set is to the document. 
% It is obtained by applying a MLP over the final hidden state of [CLS] when pre-training.

% Similar to BERT, PROP also adopts the MLM~\cite{} objective as one of its pre-training objectives to build good contextual representations for the query and the document. 
% Specifically, the MLM loss $\mathcal{L}_{MLM}$ is defined as: 
% \begin{equation}\label{mlm}
% \begin{aligned}
% \mathcal{L}_{MLM} = -\sum_{\hat{x}\in m(\textbf{x})} \log p(\hat{x}|\textbf{x}_{\backslash m(\textbf{x})}),
% \end{aligned}
% \end{equation}
% where $\textbf{x}$ denotes the input sentences, $m(x)$ and $\textbf{x}_{\backslash m(\textbf{x})}$ denotes the masked words and the rest words from $\textbf{x}$, respectively.  




\subsection{Dense Retrieval}

With the development of pre-trained language representation models, dense retrieval which is based on the low-dimensional dense representations shows great advantages over the traditional lexical matching models like BM25~\cite{}.
By matching the query and the document in the semantic latent space, dense retrieval avoids the vocabulary mismatch problem caused by the exact matching~\cite{}.
Dense retrieval provide new possibilities to replace the traditional lexical matching models that based on the inverted list.



The representation-focused bi-encoder model architecture is adopted for dense retrieval models.
Given a query $q$ and a document $d$, a pre-trained language model $PTM$ is taken as the encoder.
$q$ and $d$ are first encoded into dense representation separately, and then compute the relevance score using a simple similarity function:
\begin{equation}
    score = f(PTM(q), PTM(d)),
\end{equation}
where $f$ can be cosine and dot-product in dense retrieval.
After training is done, the whole document corpus $\mathcal{D}$ can be pre-computed and indexed.
During online stage, we can only encode queries and perform similarity search on the dense representations of the whole corpus.
As we can see, computing the relevance between $q$ and $d$ is based on their dense representations via very simple functions which has very low capacities.
The performance is totally determined by the quality of the dense representations of $q$ and $d$.
Therefore, a good universal document representation is crucial for dense retrieval.

\subsection{Autoencoder-based Language Models}

% \subsection{Contrastive learning}
% By contrasting positive pairs against negative pairs, contrastive learning has achieved great success on unsupervised representation learning in both CV and NLP.
% Specifically, the basic idea of contrastive learning is to pull the semantically close neighbors together and push apart the non-neighbors in a semantic latent space.
% This is achieved by the contrastive loss function.
% We introduce three critical component of contrastive learning framework, including  positive pairs construction, model architecture and the contrastive loss function.


% \subsubsection{Positive Pairs Construction}
% Suppose a mini-batch which is contained $N$ examples is sampled from the corpus, and then data augmentation techniques are applied to each example twice to obtain two augmented examples as a positive pair, resulting in $2N$ examples.
% In CV, the data augmentation techniques such as random cropping, random color distortions and so on have been widely used and proved to be very useful for unsupervised vision representation learning~\cite{Chen2020ASF}.
% In NLP, some researchers have also explored data augmentation techniques on sentences like random crop, delete or replace some words, apply dropout on the same sentence twice~\cite{Gao2021SimCSESC}, random mask on the embedding space~\cite{Yan2021ConSERTAC} and etc.
% We show that these techniques designed for short sentences are usually not suitable for long documents.


% \subsubsection{Model architecture}
% A neural encoder $E$ extracts representation vectors from augmented data examples.
% A general form is to take the same encoder to every example, and there are also some alternatives like an asymmetric model which don't share the encoder for two views of one example~\cite{moco}.
% Studies have been shown that introducing a learnable nonlinear $projector$ between the representation and the contrastive loss substantially improves the quality of the learned representations.
% Suppose $x_i$ is a example in the mini-batch, the representation of $x_i$ is obtained as follows:
% \begin{equation}
%     z_i = projector(E(x_i)),
% \end{equation}
% where $projector$ uses a MLP with one hidden layer and a non-linear function.



% \subsubsection{Contrastive Loss Function}

% Following Chen et.al.~\cite{Chen2020ASF}, let $z_i$ and $z_j$ be the representations of a positive pair examples in a sampled mini-batch which contain $2N$ augmented examples.
% The other $2(N-1)$ examples in the same mini-batch are treated as negatives.
% The contrastive loss function is defined as follows:
% \begin{equation}\label{ctl_loss}
%     \mathcal{L}_i = -log \frac{exp(sim(z_i, z_j)/\tau)}{\sum_{j=1}^{2N}{\mathbbm{1}_{[i\neq{j}]}exp(sim(z_i, z_j)/\tau)}},
% \end{equation}
% where $sim$ denotes the similarity function like cosine or dot-product, $\mathbbm{1}_{[i\neq{j}]} \in {0, 1}$ is an indicator function evaluating to 1 if $i \neq{j} $, and $\tau > 0$ denotes the temperature hyper-parameter.


